Summary: Chicago Quantum Exchange (CQE) Pulse-level Quantum Control Workshop

Quantum information processing holds great promise for pushing beyond the current frontiers in computing. Specifically, quantum computation promises to accelerate the solving of certain problems, and there are many opportunities for innovation based on applications in chemistry, engineering, and finance. To harness the full potential of quantum computing, however, we must not only place emphasis on manufacturing better qubits, advancing our algorithms, and developing quantum software. To scale devices to the fault tolerant regime, we must refine device-level quantum control. On May 17-18, 2021, the Chicago Quantum Exchange (CQE) partnered with IBM Quantum and Super.tech to host the Pulse-level Quantum Control Workshop. At the workshop, representatives from academia, national labs, and industry addressed the importance of fine-tuning quantum processing at the physical layer. The purpose of this report is to summarize the topics of this meeting for the quantum community at large.

==> sections/3a_quantum_hardware_backup.tex <==
\section{Quantum Hardware}
\label{Hardware}


\subsection{Physical Qubits}
\label{Physical Qubits}

Even if the theory is well defined, information must have a physical realization for computation to occur. Currently, a variety of quantum technologies can encode logical qubits within different media. We call a physical implementation of a radix-2 unit of information a physical qubit. Since today's quantum devices lack error correction, each logical qubit within an algorithm is implemented with one physical qubit in a machine. These devices, sometimes called Noisy Intermediate Scale Quantum (NISQ) devices, are error prone and are up to hundreds of qubits in size~\cite{preskill2018quantum}. Some physical qubit examples include energy levels within superconducting circuits~\cite{arute2019quantum,havlivcek2019supervised,jurcevic2021demonstration}, ions trapped by surrounding electrodes~\cite{nam2020ground,wright2019benchmarking,zhang2017observation}, neutral atoms held with optical tweezers~\cite{levine2019parallel,bernien2017probing}, and photons travelling through free space or waveguides~\cite{o2009photonic,knill2001scheme}. Each of these platforms have their unique strengths, but none has become the obvious choice for the standard quantum computing platform. 

\subsection{Physical Architectural Constraints}

Although many promising quantum technologies exist, they are imperfect and demonstrate attributes that prevent scaling in the near-term. For example, quantum state preparation, gate evolution, and measurement all are characterized by nontrivial infidelity rates and must be implemented with a limited set of instructions that depend on the control signals that are available for a specific qubit technology. Additionally, restricted \textit{connectivity} among device qubits is a key limiting factor. Qubit-qubit interaction is necessary for quantum entanglement, but unfortunately, many of today's QCs are limited in the number of qubits that are able to interact directly. Even with technologies that allow for all-to-all connectivity, such as with trapped ions, QCs are limited by the total number of qubits that are actively used during computation~\cite{pino2021demonstration}. Careful design of qubit layout on devices as well as intelligent algorithm mappers and compilers can assist with qubit communication overheads.

Qubit communication is required for quantum algorithms, but unintended communication, or \textit{crosstalk}, can cause errors during computation. Crosstalk errors experienced during quantum algorithm execution often arise from simultaneously stimulating two neighboring qubits. If the qubits are strongly coupled and ``feel'' each other, the fidelity of the two simultaneous computations can decrease. Fortunately, qubit crosstalk errors are systematic. Once identified, sources of crosstalk can be mitigated with software~\cite{murali2020software,ding2020systematic} or with improved device design~\cite{chamberland2020topological}.

Today's qubits are extremely sensitive, and as a result, crosstalk with neighboring qubits is not the only accidental signal interference that must be considered for quantum systems. Qubits also tend to couple with their surrounding environment, causing quantum information to \textit{decohere}. Amplitude damping and dephasing cause qubit decoherence errors. Amplitude damping describes the loss of energy from $\ket{1}$ to $\ket{0}$, and $T_1$ is used to denote the exponential decay time from an excited qubit state to a ground state. Dephasing error refers to the gradual loss of phase between $\ket{0}$ to $\ket{1}$ and is described by the time $T_2$. Quantum decoherence sets rigid windows for compute time on current QCs. If the qubit runtime, or period spanning the first gate up until measurement, surpasses the QC $T_1$ or $T_2$ time, the final result of computation may resemble a random distribution rather than the correct output.  

\subsection{Superconducting Circuits - A Case Study on Progress}

Superconducting circuits have emerged as a leading physical qubit implementation~\cite{majer2007coupling}. IBM has dedicated much research to the development of the Transmon-based superconducting QC, and since 2016, the company has allowed their prototype devices to be used by the public via the IBM Quantum Experience~\cite{IBMQE}. Since 2016, IBM QCs have increased from 5 to 127 qubits~\cite{heavy-hex-blog}. The significance of increasing the number of qubits on-chip to a total of $n$ is that more complex algorithms can be run that explore an exponentially larger state space, dimension $2^n$. Although the debut of larger QCs with over a hundred qubits is an impressive engineering development, limited fidelity, qubit communication, and coherence times prohibit these devices from reliably executing circuits that require all of a device's physical qubits to work in synergy.

Progress in quantum hardware is not measured simply by the consistency and count of device qubits. The gate error must also be considered as it influences the depth of circuits that a QC can run. IBM QCs have seen the average two-qubit infidelity decrease in magnitude from order $10^{-2}$ to $10^{-3}$ over the last five years~\cite{heavy-hex-blog}. Quality of multi-qubit gates is an important metric to consider when rating a QC because it enables the entanglement required for many quantum algorithms to demonstrate advantage. The importance of device size, qubit quality, and operation success is clear, thus, improving quantum systems as a whole requires a multi-targeted approach. To assist with scaling into more robust devices, IBM developed a metric referred to as Quantum Volume (QV) that aims to benchmark quantum hardware in the near term. QV is a scalar value, where higher is better, that assesses the largest random circuit of equal width and depth equal to $m$ that a QC can successfully run~\cite{cross2019validating}. As QV$=2^m$, the metric provides perspective on system performance as a general purpose QC. Capability in terms of coherence, calibration, state initialization, gate fidelity, crosstalk, and measurement quality are all captured by QV. QV is also influenced by design aspects such as chip topology, compilation tools, and basis gate set.

Recently, IBM extended the QC frontier to achieve a QV of 64, and then later 128, through the combined application of improved compiler optimizations, shorter two-qubit gates, excited state promoted readout, higher-accuracy state discrimination and open-loop correction via dynamical decoupling~\cite{jurcevic2021demonstration,IBMQS}. These breakthroughs were accompished on 27 qubit devices, demonstrating that the compute power of a quantum system is heavily influenced on compilation and low-level control; it does not depend on qubit count alone. Quantum compilation and low-level control will be discussed further in Section~\ref{software}. By focusing research to innovate in these domains, along with making developments in other areas of QC architecture, IBM anticipates to scale QCs to one million qubits and beyond~\cite{roadmap-IBM}.


